The Galactic Center Black Hole Laboratory

The super-massive 4 million solar mass black hole Sagittarius~A* (SgrA*) shows flare emission from the millimeter to the X-ray domain. A detailed analysis of the infrared light curves allows us to address the accretion phenomenon in a statistical way. The analysis shows that the near-infrared flare amplitudes are dominated by a single state power law, with the low states in SgrA* limited by confusion through the unresolved stellar background. There are several dusty objects in the immediate vicinity of SgrA*. The source G2/DSO is one of them. Its nature is unclear. It may be comparable to similar stellar dusty sources in the region or may consist predominantly of gas and dust. In this case a particularly enhanced accretion activity onto SgrA* may be expected in the near future. Here the interpretation of recent data and ongoing observations are discussed.

==> text.tex <==

The Galactic Center Black Hole Laboratory

In this article we summarize contributions on the Galactic Center, held at 
the conference 'Equations of Motion in Relativistic Gravity' at the 
Physikzentrum Bad Honnef, Bad Honnef, Germany, (February 17-23, 2013)
and the COST action MP0905 - "Black Holes in a Violent Universe" - Galactic Center  
GC2013 conference titled 'The Galactic Center Black Hole Laboratory' held
at the Instituto de Astrofisica de Andalucia (IAA-CSIC) in Granada, Spain 
(November 19 - 22, 2013).


30 pages - 7 figures -
accepted for publication by Springer's  "Fundamental Theories of Physics" series


Eckart, A., Britzen, S., Valencia-S., M., Straubmeier, C., Zensus, J.A., Karas, V., Kunneriath, D., Alberdi, A., Sabha, N., Sch\"odel, R., Puetzfeld, D. 

The super-massive 4 million solar mass black hole Sagittarius~A* (SgrA*) shows 
flare emission from the millimeter to the X-ray domain. 
A detailed analysis of the infrared light curves allows us to 
address the accretion phenomenon in a statistical way.
The analysis shows that the near-infrared flare amplitudes 
are dominated by a single state power law, with the low states 
in SgrA* limited by confusion through the unresolved stellar background.
There are several dusty objects in the immediate vicinity  of SgrA*. 
The source G2/DSO is one of them. Its nature is unclear. 
It may be comparable to similar stellar dusty sources in the region or may 
consist predominantly of gas and dust.
In this case a particularly enhanced accretion activity onto SgrA* 
may be expected in the near future. Here the interpretation of recent
data and ongoing observations are discussed.

